Debiasing Sequential Recommendation with Time-aware Inverse Propensity Scoring

Sequential Recommendation (SR) predicts users next interactions by modeling the temporal order of their historical behaviors. Existing approaches, including traditional sequential models and generative recommenders, achieve strong performance but primarily rely on explicit interactions such as clicks or purchases while overlooking item exposures. This ignorance introduces selection bias, where exposed but unclicked items are misinterpreted as disinterest, and exposure bias, where unexposed items are treated as irrelevant. Effectively addressing these biases requires distinguishing between items that were "not exposed" and those that were "not of interest", which cannot be reliably inferred from correlations in historical data. Counterfactual reasoning provides a natural solution by estimating user preferences under hypothetical exposure, and Inverse Propensity Scoring (IPS) is a common tool for such estimation. However, conventional IPS methods are static and fail to capture the sequential dependencies and temporal dynamics of user behavior. To overcome these limitations, we propose Time aware Inverse Propensity Scoring (TIPS). Unlike traditional static IPS, TIPS effectively accounts for sequential dependencies and temporal dynamics, thereby capturing user preferences more accurately. Extensive experiments show that TIPS consistently enhances recommendation performance as a plug-in for various sequential recommenders. Our code will be publicly available upon acceptance.

==> tables/pseudocode.tex <==
\begin{algorithm}[h]
\caption{Debiasing with TIPS}
\label{pesudo}
\begin{algorithmic} % 不显示行号
\Require Training set $\mathcal{D}_{\text{train}}=\{(v,t)\}$, learning rate $\eta$
\Ensure Model parameters $\varphi,\theta$
\State Initialize $\varphi,\theta$ 
\For{$\text{epoch} = 1 \to E$}
\State For each item-time pair $(v_i,t_i)\in\mathcal{D}_{\text{train}}$, obtain embeddings $\mathbf{c}_i$, $\mathbf{e}_i$ for $v_i$, $\mathbf{t}_i$ for $t_i$
\State Obtain historical interaction sequence embedding $\mathbf{S}$
\State Obtain counterfactual exposure samples $(\mathbf{e}^{sim}_i, \mathbf{t}_i)$, $(\mathbf{e}^{pop}_i, \mathbf{t}_i)$, $(\mathbf{e}_i, \mathbf{t}^*_i)$
\State Compute exposure aware sequence $\mathbf{\hat{S}}$%$\mathbf{\hat{S}}\leftarrow\operatorname{CrossAttn}(\mathbf{e}_i, \mathbf{t}_i, \mathbf{S})$
\LineComment{Modeling $\mathbf{E}\rightarrow\mathbf{C}$}
\State $\mathcal{E}^+\leftarrow\{(\mathbf{e}_i, \mathbf{t}_i),(\mathbf{e}^{sim}_i, \mathbf{t}_i)$, $(\mathbf{e}^{pop}_i, \mathbf{t}_i)$, $(\mathbf{e}_i, \mathbf{t}^*_i)\}$
\State $\mathcal{E}^-\leftarrow$ randomly sampled from $\mathcal{D}_{\text{train}\backslash\mathcal{E}^+}$
\State Compute the time-aware propensity score $s\leftarrow \pi^t(\cdot)$ for each item-time pair $(\mathbf{e},\mathbf{t})\in\mathcal{E}^{+}\cup\mathcal{E}^{-}$
% \State Calculate the time-aware propensity score $s_{v_i, t_i}$, $s_{v^{sim}_i, t_i}$, $s_{v^{pop}_i},t_i$, $s_{v_i, t^*_i}$ for $(\mathbf{e_i}, \mathbf{t}_i)$, $(\mathbf{e}^{sim}_i, \mathbf{t}_i)$, $(\mathbf{e}^{pop}_i, \mathbf{t}_i)$, $(\mathbf{e}_i, \mathbf{t}^*_i)$
\State Compute $\mathcal{L}_{EP}(\mathcal{E}^{+}, \mathcal{E}^-)$
\LineComment{Modeling $\mathbf{E}\rightarrow\mathbf{U}$}
\State $\mathcal{C}^{+}\leftarrow\{(\mathbf{e}_i, \mathbf{t}_i)\}$
\State $\mathcal{C}^{-}\leftarrow\{(\mathbf{e}^{sim}_i, \mathbf{t}_i)$, $(\mathbf{e}^{pop}_i, \mathbf{t}_i)$, $(\mathbf{e}_i, \mathbf{t}^*_i)\}$
\State Compute recommendation score $y_i\leftarrow g_\theta(\cdot)$ for each item-time pair $(\mathbf{e},\mathbf{t})\in\mathcal{C}^{+}\cup\mathcal{C}^{-}$
\LineComment{Adjust Recommendations}
  \State Compute $\mathcal{L}_{TIPS}(\mathcal{C}^+, \mathcal{C}^-, s)$
  \State Compute $\mathcal{L}\leftarrow\mathcal{L}_{EP}+\gamma\mathcal{L}_{TIPS}$
\State Update parameters $\varphi, \theta \gets \varphi, \theta - \eta \nabla_{\varphi,\theta} L$
\EndFor
\State \Return $\varphi,\theta$
\end{algorithmic}
\end{algorithm}
